Bits for Privacy: Evaluating Post-Training Quantization via Membership Inference

Deep neural networks are widely deployed with quantization techniques to reduce memory and computational costs by lowering the numerical precision of their parameters. While quantization alters model parameters and their outputs, existing privacy analyses primarily focus on full-precision models, leaving a gap in understanding how bit-width reduction can affect privacy leakage. We present the first systematic study of the privacy-utility relationship in post-training quantization (PTQ), a versatile family of methods that can be applied to pretrained models without further training. Using membership inference attacks as our evaluation framework, we analyze three popular PTQ algorithms-AdaRound, BRECQ, and OBC-across multiple precision levels (4-bit, 2-bit, and 1.58-bit) on CIFAR-10, CIFAR-100, and TinyImageNet datasets. Our findings consistently show that low-precision PTQs can reduce privacy leakage. In particular, lower-precision models demonstrate up to an order of magnitude reduction in membership inference vulnerability compared to their full-precision counterparts, albeit at the cost of decreased utility. Additional ablation studies on the 1.58-bit quantization level show that quantizing only the last layer at higher precision enables fine-grained control over the privacy-utility trade-off. These results offer actionable insights for practitioners to balance efficiency, utility, and privacy protection in real-world deployments.

==> tables/accu_and_auc.tex <==
\begin{figure*}[!t]
    \centering

    % 第一行
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cifar100_online_auc.pdf}
        \caption*{(a) The AUC of Online attack on CIFAR-100.}
        \label{fig:cifar100_online_fixed_AUC}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cifar100_online_accu.pdf}
        \caption*{(b) The accuracy of Online attack on CIFAR-100.}
        \label{fig:cifar100_online_fixed_accuracy}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cifar100_offline_fixed_auc.pdf}
        \caption*{(c) The AUC of Offline Fixed Variance attack on CIFAR-100.}
        \label{fig:cifar100_offline_fixed_AUC}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cifar100_offline_fixed_accu.pdf}
        \caption*{(d) The accuracy of Offline Fixed Variance attack on CIFAR-100.}
        \label{fig:cifar100_offline_fixed_accuracy}
    \end{minipage}

    \vspace{0.5cm}
    \caption{Accuracy and AUC of Online and Offline Fixed Variance Attacks on CIFAR-100. A red horizontal line represents the performance of the full-precision model. The results show that quantization can also reduce both AUC and accuracy.}
    \label{fig:acc_auc}
    \vspace{1cm}
\end{figure*}
